Faster Convergence of Stochastic Accelerated Gradient Descent under Interpolation

We prove new convergence rates for a generalized version of stochastic Nesterov acceleration under interpolation conditions. Unlike previous analyses, our approach accelerates any stochastic gradient method which makes sufficient progress in expectation. The proof, which proceeds using the estimating sequences framework, applies to both convex and strongly convex functions and is easily specialized to accelerated SGD under the strong growth condition. In this special case, our analysis reduces the dependence on the strong growth constant from $\rho$ to $\sqrt{\rho}$ as compared to prior work. This improvement is comparable to a square-root of the condition number in the worst case and address criticism that guarantees for stochastic acceleration could be worse than those for SGD.

==> macros/plots.tex <==
%% Plotting macros for LaTex Projects 
%% Maintainer: Aaron Mishkin <amishkin@cs.stanford.edu>


%% Tikz and PGFplots packages
\usepackage{tikz}
\usepackage{pgfplots}

% tikz and PGFplots libraries
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}



%% tikz settings 
\tikzset{
    font={\fontsize{12pt}{12}\selectfont},
}

%% PGFplots settings 
\pgfplotsset{
    % version compatibility
    compat=1.5.1,
    % basic line-styles
    primary/.style={color=black, style=solid, line width=1.5pt}, 
    secondary/.style={color=red, style=solid, line width=1.5pt}, 
}


==> macros/tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	/62f0144/
\\Dim	math.tex	/^\\newcommand{\\Dim}{\\text{Dim}}$/;"	C
\\E	math.tex	/^\\newcommand{\\E}{\\bbE}$/;"	C
\\Ek	math.tex	/^\\newcommand{\\Ek}{\\bbE_{\\zk}}$/;"	C
\\Lk	math.tex	/^\\newcommand{\\Lk}{L_{\\zk}}$/;"	C
\\Lmax	math.tex	/^\\newcommand{\\Lmax}{L_{\\text{max}}}$/;"	C
\\Lmin	math.tex	/^\\newcommand{\\Lmin}{L_{\\text{min}}}$/;"	C
\\Null	math.tex	/^\\newcommand{\\Null}{\\text{Null}}$/;"	C
\\R	math.tex	/^\\newcommand{\\R}{\\mathbb{R}}$/;"	C
\\Var	math.tex	/^\\newcommand{\\Var}[1]{\\textbf{Var}\\sbr{#1}}$/;"	C
\\Z	math.tex	/^\\newcommand{\\Z}{Z}$/;"	C
\\abr	math.tex	/^\\newcommand{\\abr}[1]{\\left\\langle#1\\right\\rangle}$/;"	C
\\abs	math.tex	/^\\newcommand{\\abs}[1]{\\left\\vert #1\\right\\vert}$/;"	C
\\addnumber	math.tex	/^\\newcommand{\\addnumber}{\\addtocounter{equation}{1}\\tag{\\theequation}}$/;"	C
\\alphak	math.tex	/^\\newcommand{\\alphak}{\\alpha_{k}}$/;"	C
\\alphakk	math.tex	/^\\newcommand{\\alphakk}{\\alpha_{k+1}}$/;"	C
\\argdot	math.tex	/^\\newcommand{\\argdot}{{\\,\\vcenter{\\hbox{\\tiny$\\bullet$}}\\,}} %generic argument dot$/;"	C
\\as	math.tex	/^\\newcommand{\\as}[1]{\\stackrel{\\text{\\rm\\tiny a.s.}}{#1}}$/;"	C
\\aside	paragraph.tex	/^\\newcommand{\\aside}[1]{(\\textcolor{red}{\\textbf{Aside}: #1})}$/;"	C
\\betak	math.tex	/^\\newcommand{\\betak}{\\beta_{k}}$/;"	C
\\betakk	math.tex	/^\\newcommand{\\betakk}{\\beta_{k+1}}$/;"	C
\\biggmid	math.tex	/^\\newcommand{\\biggmid}{\\bigg \\vert }$/;"	C
\\cbr	math.tex	/^\\newcommand{\\cbr}[1]{\\left\\{#1\\right\\}}$/;"	C
\\col	math.tex	/^\\newcommand{\\col}{\\text{Col}}$/;"	C
\\dist	math.tex	/^\\newcommand{\\dist}[1]{\\stackrel{\\text{\\rm\\tiny dist}}{#1}}$/;"	C
\\dom	math.tex	/^\\newcommand{\\dom}{\\text{Dom}}$/;"	C
\\eR	math.tex	/^\\newcommand{\\eR}{\\bar{\\mathbb{R}}}$/;"	C
\\equas	math.tex	/^\\newcommand{\\equas}{\\stackrel{\\text{\\rm\\tiny a.s.}}{=}}$/;"	C
\\equdist	math.tex	/^\\newcommand{\\equdist}{\\stackrel{\\text{\\rm\\tiny dist}}{=}}$/;"	C
\\etak	math.tex	/^\\newcommand{\\etak}{\\eta_k}$/;"	C
\\etakk	math.tex	/^\\newcommand{\\etakk}{\\eta_{k+1}}$/;"	C
\\etamax	math.tex	/^\\newcommand{\\etamax}{\\eta_{\\text{max}}}$/;"	C
\\etamin	math.tex	/^\\newcommand{\\etamin}{\\eta_{\\text{min}}}$/;"	C
\\f	math.tex	/^\\newcommand{\\f}{f}$/;"	C
\\fj	math.tex	/^\\newcommand{\\fj}{f_i}$/;"	C
\\fk	math.tex	/^\\newcommand{\\fk}{f_{i_k}}$/;"	C
\\fkk	math.tex	/^\\newcommand{\\fkk}{f_{i_{(k+1)}}}$/;"	C
\\fopt	math.tex	/^\\newcommand{\\fopt}{f^*}$/;"	C
\\grad	math.tex	/^\\newcommand{\\grad}{\\nabla f}$/;"	C
\\gradk	math.tex	/^\\newcommand{\\gradk}{\\nabla f_{i_k}}$/;"	C
\\gradkk	math.tex	/^\\newcommand{\\gradkk}{\\nabla f_{i_{(k+1)}}}$/;"	C
\\halved	math.tex	/^\\newcommand{\\halved}[1]{\\frac{#1}{2}}$/;"	C
\\ind	math.tex	/^\\newcommand{\\ind}[0]{\\perp \\!\\!\\! \\perp }$/;"	C
\\into	math.tex	/^\\newcommand{\\into}{\\rightarrow}$/;"	C
\\inv	math.tex	/^\\newcommand{\\inv}[1]{\\frac{1}{#1}}$/;"	C
\\iter	math.tex	/^\\newcommand{\\iter}{k}$/;"	C
\\mumax	math.tex	/^\\newcommand{\\mumax}{\\mu_{\\text{max}}}$/;"	C
\\mumin	math.tex	/^\\newcommand{\\mumin}{\\mu_{\\text{min}}}$/;"	C
\\oracle	math.tex	/^\\newcommand{\\oracle}{\\mbox{\\( \\calO \\)}}$/;"	C
\\rbr	math.tex	/^\\newcommand{\\rbr}[1]{\\left(#1\\right)}$/;"	C
\\row	math.tex	/^\\newcommand{\\row}{\\text{Row}}$/;"	C
\\sbr	math.tex	/^\\newcommand{\\sbr}[1]{\\left[#1\\right]}$/;"	C
\\seq	math.tex	/^\\newcommand{\\seq}[1]{\\rbr{#1}}$/;"	C
\\sgc	math.tex	/^\\newcommand{\\sgc}{\\rho}$/;"	C
\\tetak	math.tex	/^\\newcommand{\\tetak}{{\\tilde{\\eta}}_{k}}$/;"	C
\\vk	math.tex	/^\\newcommand{\\vk}{v_k}$/;"	C
\\vkk	math.tex	/^\\newcommand{\\vkk}{v_{k+1}}$/;"	C
\\vspan	math.tex	/^\\newcommand{\\vspan}{\\text{Span}}$/;"	C
\\w	math.tex	/^\\newcommand{\\w}{w}$/;"	C
\\wbar	math.tex	/^\\newcommand{\\wbar}{\\bar{w}}$/;"	C
\\wgc	math.tex	/^\\newcommand{\\wgc}{\\alpha}$/;"	C
\\wk	math.tex	/^\\newcommand{\\wk}{w_k}$/;"	C
\\wkk	math.tex	/^\\newcommand{\\wkk}{w_{k+1}}$/;"	C
\\wopt	math.tex	/^\\newcommand{\\wopt}{w^*}$/;"	C
\\x	math.tex	/^\\newcommand{\\x}{x}$/;"	C
\\xbar	math.tex	/^\\newcommand{\\xbar}{\\xbar{w}}$/;"	C
\\xk	math.tex	/^\\newcommand{\\xk}{x_k}$/;"	C
\\xkk	math.tex	/^\\newcommand{\\xkk}{x_{k+1}}$/;"	C
\\xkplus	math.tex	/^\\newcommand{\\xkplus}{x_k^+}$/;"	C
\\xopt	math.tex	/^\\newcommand{\\xopt}{x^*}$/;"	C
\\y	math.tex	/^\\newcommand{\\y}{y}$/;"	C
\\yk	math.tex	/^\\newcommand{\\yk}{y_k}$/;"	C
\\ykk	math.tex	/^\\newcommand{\\ykk}{y_{k+1}}$/;"	C
\\z	math.tex	/^\\newcommand{\\z}{z}$/;"	C
\\zk	math.tex	/^\\newcommand{\\zk}{z_{k}}$/;"	C
\\zkk	math.tex	/^\\newcommand{\\zkk}{z_{k+1}}$/;"	C
macros	README.md	/^# macros$/;"	c

